Stochastic Runge-Kutta Accelerates Langevin Monte Carlo and Beyond

Sampling with Markov chain Monte Carlo methods often amounts to discretizing some continuous-time dynamics with numerical integration. In this paper, we establish the convergence rate of sampling algorithms obtained by discretizing smooth It\^o diffusions exhibiting fast Wasserstein-$2$ contraction, based on local deviation properties of the integration scheme. In particular, we study a sampling algorithm constructed by discretizing the overdamped Langevin diffusion with the method of stochastic Runge-Kutta. For strongly convex potentials that are smooth up to a certain order, its iterates converge to the target distribution in $2$-Wasserstein distance in $\tilde{\mathcal{O}}(d\epsilon^{-2/3})$ iterations. This improves upon the best-known rate for strongly log-concave sampling based on the overdamped Langevin equation using only the gradient oracle without adjustment. In addition, we extend our analysis of stochastic Runge-Kutta methods to uniformly dissipative diffusions with possibly non-convex potentials and show they achieve better rates compared to the Euler-Maruyama scheme in terms of the dependence on tolerance $\epsilon$. Numerical studies show that these algorithms lead to better stability and lower asymptotic errors.

==> nonconvex.tex <==
\section{Non-Convex Learning}

==> srk_arxiv_arXiv/abstract.tex <==
\begin{abstract}
Sampling with Markov chain Monte Carlo methods often amounts to discretizing some continuous-time dynamics with numerical integration.
In this paper, we establish the convergence rate of sampling algorithms obtained by discretizing smooth It\^o diffusions exhibiting fast Wasserstein-$2$ contraction, based on local deviation properties of the integration scheme. 
In particular, we study a sampling algorithm constructed by discretizing the overdamped Langevin diffusion with 
the method of stochastic Runge-Kutta.
For strongly convex potentials that are smooth up to a certain order, its iterates converge to the target distribution in $2$-Wasserstein distance in $\tilde{\mathcal{O}}(d\epsilon^{-2/3})$ iterations.
This improves upon the best-known rate for strongly log-concave sampling based on the overdamped Langevin equation using only the gradient oracle without adjustment. 
In addition, we extend our analysis of stochastic Runge-Kutta methods to uniformly dissipative diffusions with possibly non-convex potentials and show they achieve better rates compared to the Euler-Maruyama scheme in terms of the dependence on tolerance $\epsilon$. 
Numerical studies show that these algorithms lead to better stability and lower asymptotic errors. 
\end{abstract}



==> srk_arxiv_arXiv/discussions.tex <==
\section{Discussion}
We established convergence rates of samplings algorithm obtained by discretizing It\^o diffusions with exponential \wtwo-contraction based on local properties of numerical schemes. 
The user-friendly conditions promote one to derive rates based on the uniform orders of the local deviation.
In addition, we showed that discretizing diffusions with SRK schemes leads to improved rates in $W_2$ for both strongly convex potentials and a certain class of non-convex potentials.

Despite focusing on SRK methods, Theorem~\ref{theo:master} can be used to obtain convergence rates for other classes of schemes. 
For the underdamped Langevin diffusion, quasi-symplectic schemes that rely on Runge-Kutta-type updates can achieve mean-square order 2.0 and beyond~\cite{milstein2003quasi}. 
For general It\^o diffusions, there exist schemes of mean-square order 1.5 and beyond, using the Fourier-Legendre series to approximate the L\'evy area~\cite{kuznetsov2018explicit}. 

Compared to some existing proofs for convergence rates in $W_2$ (e.g. \cite[Thm. 1]{cheng2017underdamped}), our Theorem~\ref{theo:master} requires two conditions (the uniform local mean and mean-square deviation bounds), neither of which can be eliminated in order to obtain a tight convergence bound. The uniform local mean deviation appears in our proof due to a direct expansion of the squared $2$-norm. This can be thought of a natural consequence of our convergence bounds being based on $W_2$. An avenue of interest is to see whether additional conditions can be identified to obtain refined bounds in $W_p$ for even integer $p > 2$.

Another direction of interest is to relax the $W_2$-contraction condition on the diffusion to $W_1$-contraction or $W_1$-decay. 
This would enable us to leverage results based on distant dissipativity, and consequently allow us to sample from a wider class of non-convex potentials~\cite{eberle2017couplings}.
Orthogonally, for the overdamped Langevin diffusion, the $W_2$-contraction condition may be relaxed to a log-Sobolev inequality condition on the target measure, if the discretization analysis is adapted to be based on the KL divergence~\cite{vempala2019rapid,raginsky2017non}. 
This would also broaden the class of non-convex potentials from which we can sample with theoretical guarantees.

Parallel to studying sampling from a mean-square convergence aspect, works in numerical analysis have established convergence results in the weak sense for SRK schemes applied to ergodic SDEs with techniques as aromatic trees and B-series~\cite{laurent2017exotic,vilmart2015postprocessed}. However, moment bounds in these works are proven by generic arguments (see e.g. \cite[Lem. 2.2.2]{milstein2013stochastic}), and reasoning about the rate's dimension dependence becomes less obvious. Refined non-asymptotic convergence bounds would provide more insight for these algorithms' performance on practical problems.

Lastly, the convergence results in $W_2$ for SRK-LD and SRK-ID can be augmented to yield generalization bounds for optimization when the excess risk is characterized using the Gibbs distribution~\cite{raginsky2017non}.

\section*{Acknowledgments}
We thank Mufan Li for insightful discussions, and
Jimmy Ba, David Duvenaud and Taiji Suzuki for helpful comments on an early draft of this work.
We also thank anonymous reviewers for helpful suggestions.
MAE is partially funded by CIFAR AI Chairs program at the Vector Institute.






==> srk_arxiv_arXiv/experiments.tex <==
\section{Numerical Simulations} \label{sec:exp}
We verify that SRK methods achieve lower asymptotic errors 
and therefore have better convergence rates. 
We sample from strongly convex potentials with SRK-LD and non-convex potentials with SRK-ID. 
In both cases, we compare with EM on $W_2$ and mean squared error (MSE) between iterates of the Markov chain and the target distribution, since our theory is based on $W_2$. We do not compare to other high-order schemes that require derivatives of the drift and diffusion coefficients.
Since directly computing $W_2$ is infeasible, we estimate it using samples instead. However sample-based estimators have a bias of order $\Omega(n^{-1/d})$~\cite{weed2017sharp}, so we perform a heuristic correction owing to the 
Sinkhorn divergence. More details on this topic can be found in Appendix~~\ref{app:bias_correction}.
Throughout this section, we fix the notation such that 
$\mathbf{1}_d$ denotes the vector of all ones, and $\lambda_{\min}(\cdot)$ and $\lambda_{\max}(\cdot)$ denote the min and max eigenvalue functions, respectively.

\subsection{Strongly Convex Potentials}


\paragraph{Gaussian Mixture.}
We consider sampling from a multivariate Gaussian mixture with density
\begin{align}
    \pi(\theta) \propto \exp \bigl(-\|\theta-a\|_{2}^{2} / 2 \bigr) + \exp \bigl(-\|\theta+a\|_{2}^{2} / 2 \bigr), \quad \theta \in \mathbb{R}^{d},
\end{align}
where $a \in \R^d$ is a parameter that measures the separation of two modes. 
As shown by~\citet{dalalyan2017theoretical}, the potential is strongly convex for $\normtwo{a}$ less than 1 
and Lipschitz smooth up to the second order. Moreover, one can verify that it is also third-order Lipschitz.
\begin{figure}[ht]
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/stepsize.pdf}} 
{
    \footnotesize
    (a) Gaussian mixture
}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/BLR-2D.pdf}} 
{
    \footnotesize
    (b) Bayesian logistic regression
}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/nonconvex-MSE-final3.pdf}}
{
    \footnotesize
    (c) Student's t regression
}
\end{minipage}
\caption{
(a) Asymptotic error in $W_2^2$ as step size increases for Gaussian mixture.
Legend has the format ``scheme (dimensionality)''.
(b) $W_2^2$ for sampling from posterior of logistic regression. 
Legend has the format ``scheme (step size)''.
(c) MSE of Bayesian inference for Student's t regression.
}
\label{fig:strongly_convex}
\end{figure}
\paragraph{Bayesian Logistic Regression.}
We consider Bayesian logistic regression (BLR)~\cite{dalalyan2017theoretical}. Given data samples $\mathrm{X} = \{x_i\}_{i=1}^n \in \R^{n \times d}$, $\mathrm{Y} = \{y_i\}_{i=1}^n \in \R^n$,
and parameter $\theta\in\R^d$, logistic regression models the Bernoulli conditional distribution with probability
$\Pr(y_i\!=\!1|x_i) = 1 / (1 + \exp(-\theta^\top x_i))$. 
We place a Gaussian prior on $\theta$ with mean zero and covariance proportional to $\Sigma^{-1}_{\mathrm{X}}$, 
where $\Sigma_{\mathrm{X}} = \mathrm{X}^\top \mathrm{X} /n$ is the sample covariance matrix. 
We sample from the posterior density
\begin{align}
    \pi(\theta)\propto \exp (-f(\theta)) =
  \exp \Big(\mathrm{Y}^\top \mathrm{X} \theta - \ssum_{i=1}^n \log(1+\exp(-\theta^\top x_i) - \tfrac{\alpha}{2}
        \| \Sigma_{\mathrm{X}}^{1/2}\theta \|_2^2 \Big).
\end{align}
As shown by~\citet{dalalyan2017theoretical}, the potential is strongly convex and Lipschitz up to the third order. 
To characterize the true posterior, we sample 100k particles driven by EM with step size $0.01$ until convergence. We subsample from these particles 1k examples to represent the true posterior each time we intend to estimate $W_2^2$. We monitor the kernel Stein discrepancy (KSD)~\cite{chwialkowski2016kernel,liu2016kernelized,gorham2017measuring} with the inverse multiquadratic kernel~\cite{gorham2017measuring} to measure the distance between the 100k particles and the true posterior. We confirm that particles faithfully approximate the true posterior with the squared KSD being less than $0.002$ in all settings. We include other details of the setup in Appendix~\ref{app:blr}.


When sampling from a Gaussian mixture and the posterior of logistic regression, we observe that SRK-LD leads to a
consistent improvement in the asymptotic error compared to EM when the same step size is used. 
In particular, Figure~\ref{fig:strongly_convex} (a) plots the asymptotic error of different step sizes for 2D and 20D Gaussian mixture problems and shows that SRK-LD is surprisingly stable for exceptionally large step sizes. 
Figure~\ref{fig:strongly_convex} (b) plots the error measured in $W_2^2$ as iteration increases for 20D BLR. 
We include additional results on sampling problems in 2D and 20D and a wall-clock time analysis in Appendix~\ref{app:additional_exp}.

\subsection{Non-Convex Potentials} \label{subsec:acc_expansion}
We consider Bayesian inference over parameters of a Student's t regression problem~\cite{gorham2016measuring}. The uninformative prior we consider is the improper uniform prior. Given samples $\mathrm{X}=\{x_i\}_{i=1}^n\in\R^{n\times d}$ and $y=\{y_i\}_{i=1}^n\in\R^n$, the posterior density is
\begin{align}
    \pi(\theta)\propto \exp (-f(\theta)) =
        \bracks{
            1+
            \bracks{
                y-\mathrm{X}\theta)^\top\Sigma^{-1}(y-\mathrm{X}\theta) / \nu
            }
        }^{-(\nu+n)/2},
\end{align}
where the degrees of freedom $\nu\in\mathbb{N}$ and covariance $\Sigma\succ 0\in\R^{n\times n}$ are parameters of the t-distribution. Since the corresponding potential is non-convex, we derive the drift coefficient as per~(\ref{eq:drift_coeff}) 
from the following diffusion coefficient:
\eq{
    \sigma(\theta) &=
        \bracks{
            1 + (y-\mathrm{X}\theta)^\top \Sigma^{-1} (y-\mathrm{X}\theta) / \nu
        }^{1/2} I_d
    .
}
One can verify that the diffusion is uniformly dissipative when 
\eq{
    \nu+n >
        \bracks{
            2\lambda_{\max}(\Sigma_{\mathrm{X}})\lambda^{-1}_{\min}(\Sigma) +
            d\lambda_{\max}(\Sigma_{\mathrm{X}})\lambda^{-1}_{\min}(\Sigma)
        } 
        \lambda_{\max}(\Sigma)\lambda^{-1}_{\min}(\Sigma_{\mathrm{X}}),
}
where $\Sigma_{\mathrm{X}} = \mathrm{X}^\top \mathrm{X} / n$ is the sample covariance matrix.
We set $n=50$, $d=2$, $\nu=2$,
$\Sigma = I_d$,
and generate data from the linear model $y_i= x_i^\top \theta_*$, where $\theta_* = \mathbf{1}_d$ and $x_i\overset{ \scriptscriptstyle\text{i.i.d.}}{\sim}\calN(0,I_d / d)$. For both EM and SRK-ID, we simulate with a step size of $10^{-3}$ initialize them from the same 2k particles approximating the stationary distribution obtained by simulating using EM with step size $10^{-6}$ until the KSD becomes less than $0.002$. We compute the MSE between the continuous-time process and the Markov chain with synchronously coupled Brownian motion. We approximate the continuous-time process by simulating using EM with step size of $10^{-6}$. 

Figure~\ref{fig:strongly_convex} (c) shows that when simulating from a good approximation to the stationary distribution with the same step size, 
the MSE of SRK-ID remains small, whereas the MSE of EM quickly diverges. This corroborates with our theory that the dependence on $\epsilon$ is better.
However, this advantage diminishes when the dimensionality increases. 
We report this observation in Appendix~\ref{app:additional_exp}. 
Notably, we do not observe any significant difference in the estimated $W_2^2$ values for the two schemes.
We suspect this is due to the discrepancy only being observable with small step sizes, and therefore the $W_2^2$ estimator would require a large sample size to have a discriminative power due to the bias.




==> srk_arxiv_arXiv/experiments_new.tex <==
\section{Examples and Numerical Studies} \label{sec:exp}
We provide examples of our theory and numerical studies showing SRK methods achieve lower asymptotic errors, are stable under large step sizes, and hence converge faster to a prescribed tolerance.
We sample from strongly convex potentials with SRK-LD and non-convex potentials with SRK-ID. 
Since our theory is in $W_2$, we compare with EM on $W_2$ and mean squared error (MSE) between iterates of the Markov chain and the target. We do not compare to schemes that require computing derivatives of the drift and diffusion coefficients.
Since directly computing $W_2$ is infeasible, we estimate it using samples instead. However, sample-based estimators have a bias of order $\Omega(n^{-1/d})$~\cite{weed2017sharp}, so we perform a heuristic correction whose description is in Appendix~\ref{app:bias_correction}.

\begin{figure}[ht]
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/stepsize.pdf}} 
{
    \footnotesize
    (a) Gaussian mixture
}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/BLR-2D.pdf}} 
{
    \footnotesize
    (b) Bayesian logistic regression
}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
\centering
{\includegraphics[width=1.0\textwidth]{figs/srk_id_dims.pdf}}
{
    \footnotesize
    (c) non-convex potential
}
\end{minipage}
\caption{
(a) Estimated asymptotic error against step size.
(b) Estimated error against number of iterations. 
(c) MSE against number of iterations.
Legends of (a) and (c) denote ``scheme (dimensionality)''.
Legend of (b) denotes ``scheme (step size)''.
}
\label{fig:strongly_convex}
\end{figure}

\subsection{Strongly Convex Potentials} \label{subsec:strongly_convex_exp}


\paragraph{Gaussian Mixture.}
We consider sampling from a multivariate Gaussian mixture with density
\eqn{
    \pi(\theta) \propto 
        \exp \bracks{- \tfrac{1}{2} \|\theta - a\|_{2}^{2} } + 
        \exp \bracks{- \tfrac{1}{2} \|\theta + a\|_{2}^{2} }, \quad \theta \in \mathbb{R}^{d},
}
where $a \in \R^d$ is a parameter that measures the separation of two modes. 
The potential is strongly convex when $\normtwo{a} < 1$ and has Lipschitz gradient and Hessian~\cite{dalalyan2017theoretical}. 
Moreover, one can verify that its third derivative is also Lipschitz.

\paragraph{Bayesian Logistic Regression.}
We consider Bayesian logistic regression (BLR)~\cite{dalalyan2017theoretical}. Given data samples $\mathrm{X} = \{x_i\}_{i=1}^n \in \R^{n \times d}$, $\mathrm{Y} = \{y_i\}_{i=1}^n \in \R^n$,
and parameter $\theta\in\R^d$, logistic regression models the Bernoulli conditional distribution with probability
$\Pr(y_i\!=\!1|x_i) = 1 / (1 + \exp(-\theta^\top x_i))$. 
We place a Gaussian prior on $\theta$ with mean zero and covariance proportional to $\Sigma^{-1}_{\mathrm{X}}$, 
where $\Sigma_{\mathrm{X}} = \mathrm{X}^\top \mathrm{X} /n$ is the sample covariance matrix. 
We sample from the posterior density
\eqn{
    \pi(\theta)\propto \exp (-f(\theta)) =
  \exp \Big(
    \mathrm{Y}^\top \mathrm{X} \theta - 
    \ssum_{i=1}^n \log( 1+\exp(-\theta^\top x_i) ) - 
    \tfrac{\alpha}{2}
        \| \Sigma_{\mathrm{X}}^{1/2}\theta \|_2^2 \Big).
}
The potential is strongly convex and has Lipschitz gradient and Hessian~\cite{dalalyan2017theoretical}. 
One can also verify that it has a Lipschitz third derivative.

To obtain the potential, we generate data from the model with the parameter $\theta_* = \mathbf{1}_d$ following~\cite{dalalyan2017theoretical,dwivedi2018log}. To obtain each $x_i$, we sample a vector whose components are independently drawn from the Rademacher distribution and normalize it by the Frobenius norm of the sample matrix $X$ times $d^{-1/2}$. 
Note that our normalization scheme is different from that adopted in~\cite{dalalyan2017theoretical,dwivedi2018log}, where each $x_i$ is normalized by its Euclidean norm.
We sample the corresponding $y_i$ from the model and fix the regularizer $\alpha = 0.3d / \pi^2$.

To characterize the true posterior, we sample 50k particles driven by EM with a step size of $0.001$ until convergence. We subsample from these particles 5k examples to represent the true posterior each time we intend to estimate squared $W_2$. We monitor the kernel Stein discrepancy~\footnote{Unfortunately, there appear to be two definitions for KSD and the energy distance in the literature, differing in whether a square root is taken or not. We adopt the version with the square root taken.} (KSD)~\cite{gorham2017measuring,chwialkowski2016kernel,liu2016kernelized} using the inverse multiquadratic kernel~\cite{gorham2017measuring} with hyperparameters $\beta=-1/2$ and $c=1$ to measure the distance between the 100k particles and the true posterior. We confirm that these particles faithfully approximate the true posterior with the squared KSD being less than $0.002$ in all settings. 

When sampling from a Gaussian mixture and the posterior of BLR, we observe that SRK-LD leads to a
consistent improvement in the asymptotic error compared to the EM scheme when the same step size is used. 
In particular, Figure~\ref{fig:strongly_convex} (a) plots the estimated asymptotic error in squared $W_2$ of different step sizes for 2D and 20D Gaussian mixture problems and shows that SRK-LD is surprisingly stable for exceptionally large step sizes. 
Figure~\ref{fig:strongly_convex} (b) plots the estimated error in squared $W_2$ as the number of iterations increases for 2D BLR. 
We include additional results on problems in 2D and 20D with error estimates in squared $W_2$ and the energy distance~\cite{szekely2003statistics} along with a wall time analysis in Appendix~\ref{app:additional_exp}.

\subsection{Non-Convex Potentials} \label{subsec:exp_nonconvex}
We consider sampling from the non-convex potential
\eqn{
    f(x) = \bigl(
            \beta + \| x \|_2^2
        \bigr)^{1/2}
        + \gamma  \log \bigl(
            \beta + \| x \|_2^2
        \bigr), \quad x \in \R^d,
}
where $\beta, \gamma > 0$ are scalar parameters of the distribution.
The corresponding density is a simplified abstraction for the posterior distribution of Student's t regression with a pseudo-Huber prior~\cite{gorham2016measuring}.
One can verify that when 
$
\text{
    \scriptsize
    $\beta + \normtwo{x}^2 < 1$
}
$ and
$
\text{
    \scriptsize
    $(4\gamma + 1) \normtwo{x}^2 < (2\gamma + 1) \sqrt{\beta + \normtwo{x}^2}$
}$, the Hessian has a negative eigenvalue. 
The candidate diffusion, where the drift coefficient is given by~\eqref{eq:drift_coeff} and diffusion coefficient
$
\text{ 
\footnotesize 
$\sigma(x) =  g(x)^{1/2} I_d$
}
$ 
with 
$
\text{
    \footnotesize
    $g(x) = \bigl( \beta + \| x \|_2^2 \bigr)^{1/2}$,
}
$ 
is uniformly dissipative if 
$
\tfrac{1}{2} -
| \gamma - \tfrac{1}{2} | \tfrac{2}{\beta^{1/2}} - 
\tfrac{d}{8 \beta^{1/2}} > 0$.
Indeed, one can verify that $\mu_1(g) \le 1$, $\mu_2(g)\le \tfrac{2}{\beta^{1/2}}$, and $\mu_1(\sigma) \le \tfrac{1}{2\beta^{1/4}}$. 
Therefore,
\eqn{
    \langle b(x) - b(y), x - y \rangle + 
    \tfrac{1}{2} \normf{\sigma(x) - \sigma(y)}^2
    \le&
        -\bigl(
            \tfrac{1}{2} -
            |\gamma - \tfrac{1}{2}| \mu_2(g) -
            \tfrac{d}{2} \mu_1(\sigma)^2
        \bigr)
        \normtwo{x - y}^2,
        \\
    \le&
        -(
            \tfrac{1}{2} -
            |\gamma - \tfrac{1}{2}| \tfrac{2}{\beta^{1/2}} - 
            \tfrac{d}{8 \beta^{1/2}}
        ) \normtwo{x - y}^2
    .
}
Moreover, $b$ and $\sigma$ have Lipschitz first two derivatives, and the latter 
satisfies the sublinear growth condition in Theorem~\ref{theo:srk_id}. 

To study the behavior of SRK-ID, we simulate using both SRK-ID and EM. 
For both schemes, we simulate with a step size of $10^{-3}$ initiated from the same 50k particles approximating the stationary distribution obtained by simulating EM with a step size of $10^{-6}$ until convergence.
We compute the MSE between the continuous-time process and the Markov chain with the same Brownian motion for $300$ iterations when we observe the MSE curve plateaus. We approximate the continuous-time process by simulating using the EM scheme with a step size of $10^{-6}$ similar to the setting in~\cite{rossler2010runge}. To obtain final results, we average across ten independent runs.
We note that the MSE upper bounds $W_2$ due to the latter being an infimum over all couplings. Hence, the MSE value serves as an indication of the convergence performance in $W_2$.

Figure~\ref{fig:strongly_convex} (c) shows that for $\beta=0.33$, $\gamma=0.5$ and $d=1$, when simulating from a good approximation to the target distribution with the same step size, the MSE of SRK-ID remains small, whereas the MSE of EM converges to a larger value. 
However, this improvement diminishes as the dimensionality of the sampling problem increases. 
We report additional results with other parameter settings in Appendix~\ref{app:srk-id_diminish}.
Notably, we did not observe significant differences in the estimated squared $W_2$ values. 
We suspect this is due to the discrepancy being dominated by the bias of our estimator. 



==> srk_arxiv_arXiv/intro.tex <==
\section{Introduction}
Sampling from a probability distribution is a fundamental problem that arises
in machine learning, statistics, and optimization. In many situations,
the goal is to obtain samples from a target distribution given only
the unnormalized density~\cite{brooks2011handbook,gelman2013bayesian,mackay2003information}.
A prominent approach to this problem is
the method of Markov chain Monte Carlo (MCMC), where an ergodic Markov chain
is simulated so that
iterates converge exactly or approximately to the distribution of interest~\cite{metropolis1953equation,brooks2011handbook}.



MCMC samplers based on numerically integrating continuous-time dynamics have proven very useful due to their ability to accommodate a stochastic gradient oracle~\cite{welling2011bayesian}.
Moreover, when used as optimizations algorithms, these methods can deliver strong theoretical guarantees in non-convex settings~\cite{raginsky2017non}.
A popular example in this regime is the unadjusted Langevin Monte Carlo (LMC) algorithm~\cite{roberts1996exponential}.
Fast mixing of LMC is inherited from exponential Wasserstein
decay of the Langevin diffusion, and numerical integration using the Euler-Maruyama scheme with a sufficiently small step size ensures the Markov chain tracks the diffusion.
Asymptotic guarantees of this algorithm are well-studied~\cite{roberts1996exponential,gelfand1991recursive,mattingly2002ergodicity},
and non-asymptotic analyses specifying explicit constants in convergence bounds were recently conducted~\cite{dalalyan2012sparse,dalalyan2017theoretical,durmus2016high,cheng2017convergence,durmus2018efficient,cheng2018sharp}.

To the best of our knowledge, the best known rate of LMC in $2$-Wasserstein distance is due to~\citet{durmus2016high} -- $\tilde{\mathcal{O}}({d}{\epsilon^{-1}})$ iterations are required to reach $\epsilon$ accuracy to $d$-dimensional target distributions with strongly convex potentials under the additional Lipschitz Hessian assumption, where $\tilde{\mathcal{O}}$ hides insubstantial poly-logarithmic factors.
Due to its simplicity and well-understood theoretical properties, LMC and its derivatives have
found numerous applications in statistics and machine learning~\cite{welling2011bayesian,ding2014bayesian}. 
However, from the numerical integration point of view,
the Euler-Maruyama scheme is usually less preferred for many problems due to its inferior stability compared to implicit schemes~\cite{anderson2009weak} and large integration error compared to high-order
schemes~\cite{milstein2013stochastic}. 






In this paper, we study the convergence rate of MCMC samplers devised from
discretizing It\^o diffusions with exponential Wasserstein-2 contraction. 
Our result provides a general framework for establishing convergence rates of existing
numerical schemes in the SDE literature when used as sampling algorithms.
In particular, we establish \textit{non-asymptotic} convergence bounds for sampling with \textit{stochastic Runge-Kutta}~(SRK) methods.
For strongly convex potentials,
iterates of a variant of SRK applied to the overdamped Langevin diffusion
has a convergence rate of $\tilde{\mathcal{O}}({d}{\epsilon^{-{2}/{3}}})$.
Similar to LMC, the algorithm only queries the gradient oracle of the potential during
each update and improves upon the best known rate of $\tilde{\mathcal{O}}({d}{\epsilon^{-1}})$
for strongly log-concave sampling 
based on the overdamped Langevin diffusion
without Metropolis adjustment, under the mild extra assumption that the potential is smooth up to the third order. 
In addition, we extend our analysis to \textit{uniformly dissipative} diffusions, which 
enables sampling from non-convex potentials by choosing a non-constant 
diffusion coefficient. We study a different variant of SRK
and obtain the convergence rate of 
$\tilde{\mathcal{O}}(d^{3/4} m^2 {\epsilon^{-1}})$
for general It\^o diffusions, where $m$ is the dimensionality of the Brownian motion.
This improves upon the convergence rate of $\tilde{\mathcal{O}}(d {\epsilon^{-2}})$
for the Euler-Maruyama scheme
in terms of the tolerance $\epsilon$, while potentially trading off dimension dependence.

Our contributions can be summarized as follows:
\vspace{-2.5mm}
\begin{itemize}[leftmargin=*,noitemsep]
\item We provide a broadly applicable theorem for establishing convergence rates of
  sampling algorithms based on discretizing It\^o diffusions exhibiting exponential Wasserstein-2 contraction to
  the target invariant measure.
  The convergence rate is explicitly expressed in terms of the contraction rate of the diffusion and 
  local properties of the numerical scheme, both of which can be easily derived.
\item We show for strongly convex potentials,
  a variant of SRK applied to the overdamped Langevin diffusion
  achieves the improved convergence rate of $\tilde{\mathcal{O}}({d}{\epsilon^{-{2}/{3}}})$
  by accessing only the gradient oracle, under mild additional smoothness conditions on the potential. 
\item We establish the convergence rate of a different variant of SRK applied
  to uniformly dissipative diffusions.
  By choosing an appropriate diffusion coefficient,
  we show the corresponding algorithm can sample from certain non-convex potentials
  and achieves the rate of $\tilde{\mathcal{O}}({d^{3/4} m^2}{\epsilon^{-1}})$.
\item We provide examples and numerical studies of sampling from both convex and non-convex potentials 
      with SRK methods and show they lead to better stability and lower asymptotic errors.
\end{itemize}

\vspace{-2mm}
\subsection{Additional Related Work}
\vspace{-1mm}



\paragraph{High-Order Schemes.}
Numerically solving SDEs has been a research area for decades~\cite{milstein2013stochastic,kloeden2013numerical}.
We refer the reader to~\cite{burrage2004numerical} for a review and to~\cite{kloeden2013numerical} for technical foundations.
\citet{chen2015convergence} studied the convergence of smooth functions evaluated at iterates of sampling algorithms obtained by discretizing the Langevin diffusion with high-order numerical schemes. 
Their focus was on convergence rates of function evaluations under a stochastic gradient oracle using asymptotic arguments. 
This convergence assessment pertains to analyzing numerical schemes in the weak sense. 
By contrast, we establish non-asymptotic convergence bounds in the $2$-Wasserstein metric, which covers a broader class of functions by the Kantorovich duality~\cite{gentil2015analogy,villani2008optimal}, and our techniques are based on the mean-square convergence analysis of numerical schemes. 
Notably, a key ingredient in the proofs by~\citet{chen2015convergence}, i.e. moment bounds in the guise of a Lyapunov function argument, is assumed without justification, whereas we derive this formally and obtain convergence bounds with explicit dimension dependent constants. 
\citet{durmus2016stochastic} considered convergence of function evaluations of schemes obtained using Richardson-Romberg extrapolation.
\citet{sabanis2018higher} introduced a numerical scheme that queries the gradient of the Laplacian based on an integrator that accommodates superlinear drifts~\cite{sabanis2019explicit}. In particular, for potentials with a Lipschitz gradient, they obtained the convergence rate of $\mathcal{\tilde{O}}({d^{4/3}}{\epsilon^{-2/3}})$. 
In optimization, high-order ordinary differential equation (ODE) integration schemes were introduced to discretize a second-order ODE and achieved acceleration~\cite{zhang2018direct}.



\vspace{-1mm}
\paragraph{Non-Convex Learning.}
The convergence analyses of sampling using the overdamped and underdamped Langevin diffusion 
were extended to the non-convex setting~\cite{cheng2018sharp,ma2019there}. 
For the Langevin diffusion, the most common assumption on the potential is strong convexity outside a ball of finite radius, in addition to Lipschitz smoothness and twice differentiability~\cite{cheng2018sharp,ma2018sampling,ma2019there}. 
More generally, \citet{vempala2019rapid} showed that convergence in the KL divergence of LMC can be derived assuming a log-Sobolev inequality of the target measure with a positive log-Sobolev constant holds. 
For general It\^o diffusions, the notion of \textit{distant dissipativity}~\cite{gorham2016measuring,eberle2016reflection,eberle2017couplings} is used to study convergence to target measures with non-convex potentials in the $1$-Wasserstein distance.
Different from these works, our non-convex convergence analysis, due to conducted in $W_2$, requires the slightly stronger uniform dissipativity condition~\cite{gorham2016measuring}.
In optimization, non-asymptotic results for stochastic gradient Langevin dynamics and its variants have been established for non-convex objectives~\cite{raginsky2017non,xu2018global,erdogdu2018global,zou2019sampling}. 

\renewcommand{\arraystretch}{1.4}
\begin{table}
\begin{center}
\caption{Convergence rates in $W_2$ for algorithms sampling from strongly convex potentials by discretizing the overdamped Langevin diffusion. ``Oracle'' refers to highest derivative used in the update. ``Smoothness'' refers to Lipschitz conditions. Note that faster algorithms exist by discretizing high-order Langevin equations~\cite{dalalyan2018sampling,cheng2017underdamped,cheng2018sharp,mou2019high,shen2019randomized} or applying Metropolis adjustment~\cite{dwivedi2018log,chen2019fast}.}
\vspace{-6mm}
\begin{tabular}[t]{ c c c c }
 \toprule
 \textbf{Method} & \textbf{Convergence Rate} & \textbf{Oracle} & \textbf{Smoothness} \\ 
 \hline
Euler-Maruyama~\cite{durmus2016high} & $\tilde{\mathcal{O}}(d\epsilon^{-2})$ & $1$st order & gradient\\
\hline
  Euler-Maruyama~\cite{durmus2016high} & $\tilde{\mathcal{O}}(d\epsilon^{-1})$ & $1$st order & gradient \& Hessian \\ 
\hline
Ozaki's~\cite{dalalyan2017theoretical}
  \tablefootnote{
  We obtain a rate in $W_2$ from the discretization analysis in KL~\cite{dalalyan2017theoretical} via standard techniques~\cite{raginsky2017non,vempala2019rapid}. }
  & $\tilde{\mathcal{O}}(d\epsilon^{-1})$ & $2$nd order & gradient \& Hessian \\
\hline
{Tamed Order 1.5~\cite{sabanis2018higher}
\tablefootnote{
\citet{sabanis2018higher} use the Frobenius norm for matrices and the Euclidean norm of Frobenius norms for 3-tensors. For a fair comparison, we convert their Lipschitz constants to be based on the operator norm.
}
} & $\tilde{\mathcal{O}}(d^{4/3}\epsilon^{-2/3})$ & $3$rd order & $1$st to $3$rd derivatives \\ 
\hline
\textbf{Stochastic Runge-Kutta~(this work)} & $ \tilde{\mathcal{O}}(d\epsilon^{-2/3})$ & $1$st order & $1$st to $3$rd derivatives \\ 
\bottomrule
\end{tabular}
\end{center}
\vspace{-6mm}
\label{table:rates}
\end{table}





==> srk_arxiv_arXiv/master_thm.tex <==
\section{Convergence Rates of Numerical Schemes for Sampling}
We present a user-friendly and broadly applicable theorem
that establishes the convergence rate of a diffusion-based sampling algorithm.
We develop our explicit bounds in the $2$-Wasserstein distance based on two crucial steps.
We first verify that the candidate diffusion exhibits exponential Wasserstein-2 contraction and thereafter 
compute the uniform local deviation orders of the scheme.
\begin{defi}[Wasserstein-$2$ rate]
A diffusion $X_t$ has Wasserstein-2 (\wtwo) rate $r:\R_{\ge 0} \to \R$ if for two instances of 
the diffusion $X_t$ initiated respectively from $x$ and $y$, we have
\eqn{
  W_2(\delta_xP_t,\delta_yP_t) 
\le r(t) \normtwo{x - y}, \quad \text{for all} \; x, y\in \R^d, t \ge 0,
}
where $\delta_xP_t$ denotes the distribution of the diffusion $X_t$ starting from $x$.
Moreover, if $r(t) = e^{- \alpha t}$ for some $\alpha >0 $, then 
we say the diffusion has exponential \wtwo-contraction. 
\end{defi}
The above condition guarantees fast mixing of the sampling algorithm.
For It\^o diffusions, uniform dissipativity suffices to ensure exponential \wtwo-contraction
$r(t) = e^{-\alpha t}$ \cite[Prop. 3.3]{erdogdu2018global}.
\begin{defi}[Uniform Dissipativity]
A diffusion defined by \eqref{eq:continuous_general} is $\alpha$-uniformly dissipative if
\eq{
    \abracks{
        b(x) - b(y), x - y
    }
    + 
    \tfrac{1}{2}\normf{\sigma(x) - \sigma(y)}^2
    \le
        -\alpha \normtwo{x-y}^2, \quad \text{for all}\; x, y \in \R^d.
}
\end{defi}
For It\^o diffusions with a constant diffusion coefficient,
uniform dissipativity is equivalent to one-sided Lipschitz continuity of the drift with coefficient $-2\alpha$.
In particular, for the overdamped Langevin diffusion \eqref{eq:continuous},
this reduces to strong convexity of the potential.
Moreover, for this special case, exponential \wtwo-contraction of the diffusion and strong convexity of the potential are equivalent~\cite{calogero2012exponential}.
We will ultimately verify uniform dissipativity for the candidate diffusions,
but we first use \wtwo-contraction to derive the convergence rate of a diffusion-based sampling algorithm.

\begin{theo}[\wtwo-rate of a numerical scheme]\label{theo:master}
  For a diffusion with invariant measure $\nu^*$, exponentially contracting $W_2$-rate $r(t) = e^{-\alpha t}$, and Lipschitz
  drift and diffusion coefficients,
  suppose its discretization based on a numerical integration scheme has uniform local deviation orders $(p_1, p_2)$ 
where $p_1 \ge {1}/{2}$ and $p_2 \ge p_1 + {1}/{2}$. 
Let $\nu_k$ be the measure associated with the Markov chain obtained from 
the discretization after $k$ steps starting from the dirac measure $\nu_0 = \delta_{x_0}$.
Then, for constant step size $h$ satisfying
\eqn{
    h < 1 
    \wedge C_h 
    \wedge \frac{1}{2\alpha}
    \wedge \frac{1}{8\mu_1(b)^2 + 8 \mu_1^{\mathrm{F}}(\sigma)^2}
    ,
}
where $C_h$ is the step size constraint for obtaining the uniform local deviation orders, 
we have
{
    \footnotesize
    \eq{
        W_2(\nu_k, \nu^*) \le 
            \bracks{
                1 - \frac{\alpha h}{2}
            }^k
            W_2(\nu_0, \nu^*)
            +
            \bracks{
                \frac{
                    8\bracks{
                        16 \mu_1(b) \lambda_1 + \lambda_2
                    }
                }{\alpha^2} +
                \frac{2 \lambda_1}{\alpha}
            }^{1/2}
            h^{p_1 - 1/2}. \label{eq:main_bound}
    }
}
Moreover, if $p_1 > 1/2$ and the step size additionally satisfies
{
\footnotesize
  \eqn{
      h <
        \bracks{
          \frac{2}{\epsilon}
              \sqrt{
                  \frac{64 ( 16 \lambda_1 \mu_1(b) + \lambda_2 ) }{\alpha^2}
                  + 
                  \frac{2 \lambda_1}{\alpha}
              }
      }^{-1 / (p_1 - 1/2)},
  }
}
then $W_2(\nu_k, \nu^*)$ converges in $\mathcal{\tilde{O}}({\epsilon^{-{1}/{(p_1 - 1/2)}}})$ iterations within a sufficiently small positive error $\epsilon$.
\end{theo}

Theorem~\ref{theo:master} directly translates mean-square order
results in the SDE literature to convergence rates of sampling algorithms in $W_2$. 
The proof deferred to Appendix~\ref{proof:master} follows from
an inductive argument over the local deviation at each step (see e.g. \cite{milstein2013stochastic}),
and the convergence is provided by the exponential \wtwo-contraction of the diffusion.
To invoke the theorem and obtain convergence rates of a sampling algorithm,
it suffices to (i) show that the candidate diffusion is uniformly dissipative
and (ii) derive the local deviation orders for the underlying discretization.
Below, we demonstrate this on both the overdamped Langevin and general It\^o diffusions when the EM scheme is used for discretization, as well as the underdamped Langevin diffusion when a linearization is used for discretization~\cite{cheng2017underdamped}. 
For these schemes, local deviation orders are either well-known or straightforward to derive. 
Thus, convergence rates for corresponding sampling algorithms can be easily obtained using Theorem~\ref{theo:master}. 


\begin{exam}
  Consider sampling from a target distribution whose potential is strongly convex using
  the overdamped Langevin diffusion \eqref{eq:continuous} discretized by the EM scheme.
  The scheme has local deviation of orders $(1.5, 2.0)$ for It\^o diffusions with
  constant diffusion coefficients
  and drift coefficients that are sufficiently smooth
  \footnote{In fact, it suffices to ensure the drift is three-times differentiable with Lipschitz gradient and Hessian.} 
  (see e.g.~\cite[Sec. 1.5.4]{milstein2013stochastic}).
  Since the potential is strongly convex,
  the Langevin diffusion is uniformly dissipative and achieves exponential \wtwo-contraction~\cite[Prop. 1]{durmus2016high}.
  Elementary algebra shows that Markov chain moments are bounded~\cite[Lem. A.2]{erdogdu2018global}. 
  Therefore, Theorem~\ref{theo:master} 
  implies that the rate of the sampling is
  $\tilde{\mathcal{O}}(d \epsilon^{-1})$, where the dimension dependence can be extracted
  from the explicit bound. This recovers the result by~\citet[Thm. 8]{durmus2016high}. 
\end{exam}

\begin{exam} \label{exam:em_unif_diss}
  If a general It\^o diffusion \eqref{eq:continuous_general}
  with Lipschitz smooth drift and diffusion coefficients
  is used for the sampling task,
  local deviation orders of the EM scheme reduce to $(1.0, 1.5)$
  due to the approximation of the diffusion term \cite{milstein2013stochastic} --
  this term is exact for Langevin diffusion.
  If we further have uniform dissipativity, 
  it can be shown that Markov chain moments are bounded \cite[Lem. A.2]{erdogdu2018global}. 
  Hence, Theorem~\ref{theo:master} concludes that the convergence rate is $\tilde{\mathcal{O}}(d \epsilon^{-2})$.
  We note that for the diffusion coefficient, we use the Frobenius norm for the 
  Lipschitz and growth constants which potentially hides dimension dependence factors. 
  The dimension dependence worsens if one were to convert all bounds to be based on the operator norm 
  using the pessimistic inequality 
  $
  \text{
    \footnotesize
    $
      \normf{\sigma(x)} \le ( d^{1/2} + m^{1/2} ) \normop{\sigma(x)}
    $
  }$.
  Appendix~\ref{app:em_unif_diss} provides a convergence bound with explicit constants.
\end{exam}

\begin{exam}
  Consider sampling from a target distribution whose potential is strongly convex using the underdamped Langevin diffusion:
  \eq{
    \dX_t &= V_t \dt, \quad
    \dV_t = - \gamma V_t \dt - u \nabla f (X_t) \dt + \sqrt{2 \gamma u} \dB_t.
  }
  \citet{cheng2017underdamped} show that the continuous-time process $\{(X_t, X_t + V_t)\}_{t 
  \ge 0}$ exhibits exponential \wtwo-contraction when the coefficients $\gamma$ and $u$ are appropriately chosen~\cite[Thm. 5]{cheng2017underdamped}. Moreover, the scheme devised by linearizing the degenerate SDE for the augmented state has uniform local deviation orders $(1.5, 2.0)$~\footnote{\citet{cheng2017underdamped} derive the uniform local mean-square deviation order. Jensen's inequality implies that the local mean deviation is of the same uniform order. This entails uniform local deviation orders are $(2.0, 2.0)$ and hence also $(1.5, 2.0)$ when step size constraint $C_h \le 1$; note $p_2 \ge p_1 + 1/2$ is required to invoke Theorem~\ref{theo:master}.}~\cite[Thm. 9]{cheng2017underdamped}. 
  Theorem~\ref{theo:master} implies that the convergence rate is $\mathcal{O}(d^{1/2} \epsilon^{-1})$, where the dimension dependence is extracted from explicit bounds. This recovers the result by~\citet[Thm. 1]{cheng2017underdamped}.
\end{exam}

Since the first version of this paper appeared on arXiv, several new schemes were devised in the literature. 
We include the example of deriving the convergence rate for the recently proposed randomized midpoint method~\cite{shen2019randomized}. This example demonstrates that Theorem~\ref{theo:master} can also be applied to schemes that include additional randomness which is independent of that of the Brownian motion.
\begin{exam}
\citet{shen2019randomized} discretize the underdamped Langevin diffusion with a variant of the midpoint method, where the midpoint is computed with the linearization scheme~\cite{cheng2017underdamped} at a random time $\tau$ uniformly selected in $[0, h]$.
It can be shown that the local mean-square deviation order is the same as that of the one-step linearization scheme~\cite[Lem. 2]{shen2019randomized}. 
However, one sees that the local mean deviation order improves by inspecting the following bound
\eqn{
\text{
\footnotesize
$
  \big\|
    \E \big [ \tV_k - V_h^{(k)} | \F_{t_{k-1}} \big]
  \big\|_2^2
  \le
  \E_{\not \tau} \big [
    \big\| 
      \E_{\tau} [ \tV_k - V_h^{(k)}]
    \big\|_2^2
    | \F_{t_{k-1}}
  \big ]
  \le
  \mathcal{O}\bracks{
    \| \tV_{k-1} \|_2^2 h^{8}
    \! + \!
    \| \nabla f(\tX_k) \|_2^2  h^{10}
    \! + \!
    h^{9}
  },
$
}
}
where $\E_\tau$ and $\E_{\not \tau}$ denote taking expectation over the random time and Brownian motion, respectively.
The first and second inequalities are respectively by Jensen's and Lemma 2 of \cite{shen2019randomized}. 
A similar improvement holds for the position variable. Combined with moment bounds, this gives uniform deviation orders of $(2, 4)$ for the augmented SDE $\{(X_t, X_t + V_t)\}_{t\ge 0}$, which implies a convergence rate of $\tilde{\mathcal{O}}(\epsilon^{-2/3})$ without high-order smoothness for sufficiently small step size.
\end{exam}

While computing the local deviation orders of a numerical scheme for a single step is often straightforward,
it is not immediately clear how one might verify them uniformly for each iteration. This
requires a uniform bound on moments of the Markov chain defined by the numerical scheme. 
As our second principal contribution, we explicitly bound the Markov chain moments of SRK schemes
which, combined with Theorem~\ref{theo:master}, leads to improved rates by only accessing the first-order oracle.



==> srk_arxiv_arXiv/nonconvex.tex <==
\section{Non-Convex Learning}

==> srk_arxiv_arXiv/prelim.tex <==
\paragraph{Notation.}
We denote the $p$-norm of a real vector $x \in \R^d$ by $\norm{x}_p$. 
For a function $f: \R^d \to \R$, we denote its $i$th derivative by $\nabla^i f(x)$ and
its Laplacian by $ \Delta f = \sum_{i=1}^d {\partial^2 f_i(x)}/{\partial x_i^2}$.
For a vector-valued function $g: \R^d \to \R^m$,
we denote its vector Laplacian by $\Vec{\Delta} (g)$, i.e. $\Vec{\Delta} (g)_i = \Delta (g_i)$.
For a tensor $ T \in \R^{d_1 \times d_2 \times \cdots \times d_m}$,
we define its operator norm recursively as $ \normop{T} = \sup_{\norm{u}_2\le1} \normop{T[u]}$,
where $T[u]$ denotes the tensor-vector product.
For $f$ sufficiently differentiable, we denote the Lipschitz and polynomial coefficients of its $i$th order derivative as
\eqn{
  \mu_{0}(f) \!=\! 
               \sup_{x \in \mathbb{R}^{d}}\|f(x)\|_{\mathrm{op}},\ \
               \mu_{i}(f)\! = 
               \!\!\!\!\!\!
               \sup_{ x, y \in \mathbb{R}^{d}, x \neq y} \!\!\!\!\!
               \tfrac{ \normop{\nabla^{i-1} f(x)-\nabla^{i-1} f(y)} }{ \normtwo{x - y}},
               \ \text{and} \ \pi_{i, n} (f) \!=\! \sup_{ x \in \R^d} \tfrac{\normop{\nabla^{i-1} f(x)}^n}{ 1 + \normtwo{x}^n},
}
with the exception in Theorem~\ref{theo:srk_id}, where $\pi_{1, n}(\sigma)$ is used for a sublinear growth condition.
We denote Lipschitz and growth coefficients under the Frobenius norm $\normf{\cdot}$ as $\mu_1^{\mathrm{F}}(\cdot)$ and $\pi_{1,n}^{\mathrm{F}}(\cdot)$, respectively.

\vspace{-1mm}
\paragraph{Coupling and Wasserstein Distance.}
We denote by $\B(\R^d)$ the Borel $\sigma$-field of $\R^d$. Given probability measures $\nu$ and $\nu'$ on $(\R^d, \B(\R^d))$, we define a coupling (or transference plan) $\zeta$ between $\nu$ and $\nu'$ as a probability measure on $(\R^d \times \R^d, \B(\R^d \times \R^d)) $ such that $\zeta(A \times \R^d) = \nu(A)$ and $\zeta(\R^d \times A) = \nu'(A)$ for all $A \in \B(\R^d)$. Let $\mathrm{couplings}(\nu, \nu')$ denote the set of all such couplings. We define the $2$-Wasserstein distance between a pair of probability measures $\nu$ and $\nu'$ as 
\eqn{
  W_2(\nu, \nu') = 
    \inf_{\zeta \in \mathrm{couplings}(\nu, \nu')} \bracks{ \sint \normtwo{x - y}^2 \dzeta(\nu, \nu') }^{1/2}.
}

\vspace{-4mm}
\section{Sampling with Discretized Diffusions}
We study the problem of sampling from a target distribution $p(x)$
with the help of a candidate It\^o diffusion~\cite{ma2015complete,meyn2012markov} given as the solution to the following stochastic differential equation (SDE):
\begin{align}
  \dX_t = b(X_t) \dt + \sigma(X_t) \dB_t, \quad  \text{with} \quad X_0 = x_0, \label{eq:continuous_general}
\end{align}
where $b: \R^d \to \R^d$ and $\sigma: \R^d \to \R^{d \times m}$ are termed as
the drift and diffusion coefficients, respectively.
Here, $\{B_t\}_{t\ge0}$ is an $m$-dimensional Brownian motion adapted to the filtration $\{\F_t\}_{t \ge 0}$, whose $i$th dimension we denote by $
\text{
  \footnotesize
  $
    \{B_t^{(i)}\}_{t\ge0}
  $
}$.
A candidate diffusion should be chosen so that
(i) its invariant measure is
the target distribution $p(x)$ and (ii) it exhibits fast mixing properties.
Under mild conditions, one can design a diffusion with the target invariant measure
by choosing the drift coefficient as (see e.g. \cite[Thm. 2]{ma2015complete})
\begin{align}
  b(x) = \tfrac{1}{2p(x)}\abracks{
  \nabla , p(x) w(x)
  } , \quad \text{where}\quad w(x) = \sigma(x) \sigma(x)^\top + c(x),  \label{eq:drift_coeff}
\end{align}
$c(x)\in \R^{d \times d}$ is any skew-symmetric matrix and $\abracks{\nabla, \cdot}$
is the divergence operator for a matrix-valued function, i.e. 
$ \abracks{\nabla, w(x)}_i = \sum_{j=1}^{d} {\partial w_{i,j}(x)}/{\partial x_j}$ for $w: \R^d \to \R^{d\times d}$.
To guarantee that this diffusion has fast convergence properties, we will require certain dissipativity conditions
to be introduced later.
For example, if the target is the Gibbs measure of a strongly convex potential $f: \R^d \to \R$,
i.e., $p(x) \propto \exp{ \bracks{- f(x)}}$, a popular candidate diffusion is
the (overdamped) Langevin diffusion which is the solution to the following SDE:
\begin{align}
    \dX_t = -\nabla f(X_t) \dt + \sqrt{2} \dB_t, \quad \text{with}\quad X_0 = x_0 \label{eq:continuous}.
\end{align}
It is straightforward to verify \eqref{eq:drift_coeff} for the above diffusion which implies that the target $p(x)$
is its invariant measure.
Moreover, strong convexity of $f$ implies uniform dissipativity and ensures that the diffusion achieves fast convergence.

\subsection{Numerical Schemes and the It\^o-Taylor Expansion}
In practice, the It\^o diffusion \eqref{eq:continuous_general} (similarly \eqref{eq:continuous})
cannot be simulated in continuous time and is instead approximated by
a discrete-time numerical integration scheme. Owing to its simplicity,
a common choice is the Euler-Maruyama (EM) scheme \cite{kloeden2013numerical},
which relies on the following update rule,
\begin{align} \label{eq:em_general}
  \tX_{k+1} = \tX_k + h\, b(\tX_k) + \sqrt{h}\, \sigma(\tX_k) \xi_{k+1}, \quad k=0, 1, \dots,
\end{align}
where $h$ is the step size and $\xi_{k+1} \overset{\text{i.i.d.}}{\sim} \N(0, I_d)$ is independent of $\tX_k$ for all $k \in \mathbb{N}$.
The above iteration defines a Markov chain and due to discretization error,
its invariant measure $\tilde{p}(x)$ is different from the target distribution $p(x)$; yet,
for a sufficiently small step size, the difference between $\tilde{p}(x)$
and $p(x)$ can be characterized (see e.g. \cite[Thm. 7.3]{mattingly2002ergodicity}).

Analogous to ODE solvers, numerical schemes such as the EM scheme and SRK schemes are derived based on approximating the continuous-time dynamics locally.
Similar to the standard Taylor expansion, It\^o's lemma induces a stochastic
version of the Taylor expansion of a smooth function evaluated at a stochastic process at time $t$.
This is known as the It\^o-Taylor (or Wagner-Platen) expansion~\cite{milstein2013stochastic}, and
one can also interpret the expansion as recursively applying It\^o's lemma to terms in the integral form of an SDE. 
Specifically, for $g:\R^d \to \R^d$, we define the operators:
\eq{
  L (g) (x) =
  \nabla g(x) \cdot b(x) \!+\! 
  \tfrac{1}{2} \ssum_{i=1}^m \nabla^2 g(x) [\sigma_i(x), \, \sigma_i(x)], 
  \quad
  \Lambda_j (g) (x) = \nabla g(x) \cdot \sigma_j (x), \label{eq:ito_taylor_ops}
}
where $\sigma_i(x)$ denotes the $i$th column of $\sigma(x)$.
Then, applying It\^o's lemma to the integral form of the SDE~\eqref{eq:continuous_general} with the starting point $X_0$ yields the following expansion around $X_0$~\cite{kloeden2013numerical,milstein2013stochastic}:
\eqn{
  \text{
    \footnotesize
    $X_t $
  }
  \!=\!&\!\! 
  \, 
  \overbrace{
    \underbrace{
      \text{
        \footnotesize
        $X_0+
        t\, b(X_0)  
        + \sigma(X_0) B_t
        $ 
      }
    }_{\text{Euler-Maruyama update}}
    +
    \text{\footnotesize
      $\ssum_{i,j=1}^m \sint_0^t \sint_0^s \Lambda_j (\sigma_i) (X_u) \!\dB_u^{(j)}\! \dB_u^{(i)}$
    }
  }^{\text{mean-square order 1.0 stochastic Runge-Kutta update}}
  + 
  \text{\footnotesize
    $\sint_0^t \sint_0^s L(b) (X_u)\!\du\! \ds$
  }
  \\&
  +
  \text{\footnotesize
    $\ssum_{i=1}^m \sint_0^t \sint_0^s L (\sigma_i) (X_u) \du \dB_s^{(i)}$
  }
  + 
  \text{
    \footnotesize
    $\ssum_{i=1}^m \sint_0^t \sint_0^s \Lambda_i (b) (X_u) \dB_u^{(i)} \ds.$
  } 
  \numberthis \label{eq:ito_taylor_expansion}
}
The expansion justifies the update rule of the EM scheme, since the discretization is 
nothing more than taking the first three terms on the right hand side of~\eqref{eq:ito_taylor_expansion}.
Similarly, a mean-square order 1.0 SRK scheme for general It\^o diffusions -- introduced in Section~\ref{subsubsec:srk-nonconvex} -- approximates the first four terms.
In principle, one may recursively apply It\^o's lemma
to terms in the expansion to obtain a more fine-grained approximation.
However, the appearance of non-Gaussian terms in the guise of iterated Brownian integrals 
presents a challenge for simulation.
Nevertheless, it is clear that the above SRK scheme will be a more accurate local approximation than the EM scheme,
due to accounting more terms in the expansion. As a result, the local deviation
between the continuous-time process and Markov chain will be smaller.
We characterize this property of a numerical scheme as follows.

\begin{defi}[Uniform Local Deviation Orders]
  Let $\{\tX_k\}_{k\in \mathbb{N}}$ denote the discretization of an It\^o diffusion $\{X_t\}_{t\ge 0}$
  based on a numerical integration scheme with constant step size $h$,
  and its governing Brownian motion $\{B_t\}_{t\ge 0}$ be adapted to the filtration $\{\F_t\}_{t \ge 0}$.
  Suppose 
  $
  \text{
    \footnotesize
    $
    \{X_s^{(k)}\}_{s\ge 0}
    $
  }
  $ is another instance of the same diffusion starting from $\tX_{k-1}$ at $s=0$
  and governed by the Brownian motion $\{B_{s+h(k-1)}\}_{s\ge 0}$. 
  Then, the numerical integration scheme has local deviation 
  $
  \text{
    \footnotesize
    $
    D_{h}^{(k)} = \tX_{k} - X_h^{(k)}
    $
  }
  $
  with uniform orders $(p_1, p_2)$ if 
  \begin{align}
    \mathcal{E}_k^{(1)}
      = \Exp{
        \mathbb{E} \big[
          \|
          D_{h}^{(k)}
          \|_2^2 | \F_{t_{k-1}}
        \big]
      } \le \lambda_1 h^{2 p_1}, \quad
    \mathcal{E}^{(2)}_k
      = \Exp{ \big\|
      \mathbb{E}\big[
      D_{h}^{(k)} | \F_{t_{k-1}}
      \big]
    \big\|_2^2 } \le 
    \lambda_2 h^{2 p_2}, \label{eq:uniform_local_deviation_orders}
  \end{align}
  for all $k \in \mathbb{N}_{+}$ and $0 \le h < C_h$, where constants $0 < \lambda_1, \lambda_2, C_h < \infty$. 
  We say that $\scriptstyle \mathcal{E}_k^{(1)}$ and $\scriptstyle \mathcal{E}_k^{(2)}$ are  
  the local mean-square deviation and the local mean deviation at iteration $k$, respectively. 
\end{defi}
In the SDE literature, local deviation orders are defined to derive the mean-square 
order (or strong order) of numerical schemes~\cite{milstein2013stochastic}, 
where the mean-square order is defined as the maximum half-integer $p$ 
such that 
$
\E [
    \| X_{t_k} - \tX_{k} \|_2^2
  ]
  \le
    C h^{2 p}
$
for 
a constant $C$ independent of step size $h$ and 
all $k \in \mathbb{N}$ where $t_k < T$.
Here, $\{X_{t}\}_{t\ge0}$ is the continuous-time process, $\tX_k (k=0,1,\dots)$  is the Markov chain 
with the same Brownian motion as the continuous-time process, and $T < \infty$ is the 
terminal time.
The key difference between our definition of \textit{uniform} local deviation orders and
local deviation orders in the SDE literature is we require the extra step of 
ensuring the expectations of $\scriptstyle \mathcal{E}_k^{(1)}$ 
and $\scriptstyle \mathcal{E}_k^{(2)}$ are bounded across all iterations,
instead of merely requiring the two deviation variables to be bounded
by a function of the previous iterate.



==> srk_arxiv_arXiv/srk.tex <==
\section{Sampling with Stochastic Runge-Kutta and Improved Rates} \label{sec:srk}
We show that convergence rates of sampling can be significantly improved if
an It\^o diffusion with exponential \wtwo-contraction is discretized using SRK methods.
% One key advantage of this class of schemes is they do not require evaluating high-order derivatives of the drift and diffusion coefficients which may be costly.
Compared to the EM scheme, SRK schemes
we consider query the same order oracle and improve on the deviation orders.
% Although SRK methods for SDEs and 
% RK methods for ODEs are both motivated by approximating the local change more accurately, 
% the formalisms of two are different due to rules of 
% calculus being different~\cite{milstein2013stochastic,rossler2010runge}. 

Theorem~\ref{theo:master} hints that one may expect the convergence rate of sampling to improve
as more terms of the It\^o-Taylor expansion are incorporated in the numerical integration scheme. 
% any discretization which includes high-order terms in the It\^o-Taylor expansion that satisfies the local deviation conditions suffices improve the convergence rate. 
However, in practice, 
% the number of terms in the expansion doubles each time as one attempts to apply the operators $L$ and $\Lambda$. Yet, 
a challenge for simulation is the appearance of non-Gaussian terms in the form of iterated It\^o integrals.  
% These terms are difficult to simulate exactly and are costly to approximate accurately. 
Fortunately, since the overdamped Langevin diffusion has a constant diffusion coefficient, efficient 
SRK methods can still be applied to accelerate convergence.

\subsection{Sampling from Strongly Convex Potentials with the Langevin Diffusion}
% \murat{Refer to Ito-taylor expansion, give intuition on SRK}
We provide a non-asymptotic analysis for integrating the overdamped Langevin diffusion based on a
mean-square order 1.5 SRK scheme for SDEs with constant diffusion coefficients~\cite{milstein2013stochastic}. 
We refer to the sampling algorithm as SRK-LD. Specifically, given a sample from the previous iteration $\tX_k$, 
\begin{align}
    \tH_1 &= \tX_k + \sqrt{2h} \sbracks{
        \bracks{
            \frac{1}{2} + \frac{1}{\sqrt{6}}
        } \xi_{k+1} + 
        \frac{1}{\sqrt{12}} \eta_{k+1}
    } , \notag \\
    \tH_2 &= \tX_k - h \nabla f(\tX_k) + \sqrt{2h} \sbracks{
        \bracks{
            \frac{1}{2} - \frac{1}{\sqrt{6}}
        } \xi_{k+1} + 
        \frac{1}{\sqrt{12}} \eta_{k+1}
    }, \notag \\
    \tX_{k+1} &= \tX_k -
    \frac{h}{2} \bracks{
        \nabla f(\tH_1) +
        \nabla f(\tH_2)
    } 
    + \sqrt{2h} \xi_{k+1} 
    % \quad  \xi_{k+1}, \eta_{k+1} \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, I_d) 
    \label{eq:srk},
\end{align}
where $h$ is the step size and $\xi_{k+1}, \eta_{k+1} \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, I_d)$ are independent of $\tX_k$ for all $k\in\mathbb{N}$. We refer the reader to~\cite[Sec. 1.5]{milstein2013stochastic} for a detailed derivation of the scheme and other background information.

% The algorithm is derived from the following update equations for $t = kh + \delta$ and $\delta \in [0,h]$,
% \begin{align}
%     X_{t}^{(1)} &= X_{kh} + \sqrt{2} \sbracks{
%         \frac{1}{\delta} \int_{kh}^{t} \int_{kh}^s \dB_u \ds + 
%         \frac{1}{\sqrt{6}} \int_{k h}^{t} \dB_s
%     }, \notag \\
%     X_{t}^{(2)} &= X_{kh} - \nabla f(X_{kh}) \delta + \sqrt{2} \sbracks{
%         \frac{1}{\delta} \int_{kh}^{t} \int_{kh}^s \dB_u \ds -
%         \frac{1}{\sqrt{6}} \int_{k h}^{t} \dB_s
%     }, \notag \\
%     X_{t} &= X_{kh} - \bracks{
%         \nabla f(X_{t}^{(1)}) +
%         \nabla f(X_{t}^{(2)})
%     } \frac{\delta}{2} + \sqrt{2} \int_{kh}^{t} \dB_s \label{eq:srk_integral_form}.
% \end{align}
% where
% $$\Psi_{kh}(t) = \int_{kh}^{t} \int_{kh}^s \dB_u \ds.$$
% \begin{proof}
% By It\^o's Lemma,
% \begin{align}
%     \dtX_t^{(1)} &= \sqrt{2} \bracks{
%         - \frac{1}{\delta^2} \Psi(t) \dt 
%         + \frac{1}{\delta} B_t \dt
%         + \frac{1}{\sqrt{6}} \dB_t
%     }, \notag \\
%     \dtX_t^{(2)} &= 
%     -\nabla f(X_{kh}) \dt +
%     \sqrt{2} \bracks{
%         - \frac{1}{\delta^2} \Psi(t) \dt 
%         + \frac{1}{\delta} B_t \dt
%         - \frac{1}{\sqrt{6}} \dB_t
%     }.
% \end{align}
% Thus, 
% \begin{align}
%     \dee \nabla f(X_t^{(1)}) =&
%     \sqrt{2} \abracks{
%         \nabla^2 f(X_t^{(1)}), -\frac{1}{\delta^2} \Psi(t) + \frac{1}{\delta} B_t
%     } \dt + 
%     \frac{1}{\sqrt{3}} \abracks{
%         \nabla^2 f(X_t^{(1)}), \dB_t
%     } \notag \\
%     &+ \frac{1}{6}\Delta(\nabla f) (X_t^{(1)}) \dt \\
%     \dee \nabla f(X_t^{(2)}) =&
%     - \abracks{\nabla^2 f(X_t^{(2)}), \nabla f(X_t^{(2)})} \dt +
%     \sqrt{2} \abracks{
%         \nabla^2 f(X_t^{(2)}), -\frac{1}{\delta^2} \Psi(t) + \frac{1}{\delta} B_t
%     } \dt \notag \\
%     &- \frac{1}{\sqrt{3}} \abracks{
%         \nabla^2 f(X_t^{(2)}), \dB_t
%     } +
%     \frac{1}{6}\Delta(\nabla f) (X_t^{(2)}) \dt.
% \end{align}
% Let $e_t = X_t - X_t$, then
% \begin{align}
%     \de_t = 
%     -\nabla f(X_t) \dt +
%     \frac{1}{2} \bracks{
%         \nabla f(X_t^{(1)}) + f (X_t^{(2)}) 
%     } \dt + 
%     \frac{\delta}{2} \bracks{
%         \dee \nabla f(X_t^{(1)}) + 
%         \dee \nabla f(X_t^{(2)})
%     }
% \end{align}
% By It\^o's Lemma, 
% \begin{align}
%     \norm{e_t}^2 - \norm{e_{kh}}^2 = \int_{kh}^t \abracks{
%         e_s, \de_s
%     } +
%     \int_{kh}^t \de_s^2.
% \end{align}
% Hence, 
% \begin{align}
%     \frac{\dee }{\dee t} \Exp{
%         \norm{e_t}^2 | \mathcal{F}_{kh}
%     } = \abracks{
%     }
% \end{align}
% \end{proof}
% \murat{Fix orders below.}
\begin{theo}[SRK-LD] \label{theo:srk_ld}
Let $\nu^*$ be the target distribution
with a strongly convex potential that is four-times differentiable with Lipschitz continuous
first three derivatives.
Let $\nu_k$ be the distribution of the $k$th Markov chain iterate
defined by \eqref{eq:srk} starting from the dirac measure $\nu_0 = \delta_{x_0}$.
Then, for a sufficiently small step size,
% there exists a constant $C_{\mathrm{LD}}$ such that for uniform step size $h < C_{\mathrm{LD}}$,
1.5 SRK scheme has uniform local deviation orders $(2.0, 2.5)$, and 
$W_2(\nu_k, \nu^*)$ converges within $\epsilon$ error in $\tilde{\mathcal{O}}(d \epsilon^{-2/3})$
iterations.
\end{theo}
The proof of this theorem is given in Appendix~\ref{app:srk_ld} where we provide explicit constants. 
The basic idea of the proof
is to match up the terms in the It\^o-Taylor expansion to terms in the Taylor expansion 
of the discretization scheme. However, extreme care is needed to ensure a tight dimension dependence. 

% new stuff regarding stochastic grad
% v1
% \subsubsection{Convergence Under an Unbiased Stochastic Oracle}
% For large-scale applications, computing full gradients during each iteration can become costly. Fortunately, for SRK-LD, the convergence rate is retained when we replace the exact first-order oracle with an unbiased stochastic one, provided queries of the latter have a variance not overly large.
% \begin{theo}
% Consider replacing the full-gradient in~\eqref{eq:srk} with an unbiased stochastic gradient $\hat{\nabla} f$ such that $\E[ \hat{\nabla} f(x) - \nabla f(x)] = 0$ and $\E[ \| \hat{\nabla} f(x) - \nabla f(x) \|^2 ] \le d \sigma^2$ for all $x \in \R^d$. Then, $W_2(\nu_k, \nu^*)$ converges within $\epsilon$ error in $\tilde{\mathcal{O}}(d \epsilon^{-2/3})$, if .
% \end{theo}

% % v2
\begin{remark}
For large-scale Bayesian inference, computing the full gradient of the potential can be costly. 
Fortunately, for SRK-LD, the convergence rate is retained when we replace the first-order oracle with an unbiased stochastic one, provided queries of the latter have a variance not overly large. 
We provide an informal discussion in Appendix~\ref{app:srk-ld-stochasticgrad}.
\end{remark}

% before:
% We emphasize that 1.5 SRK scheme \eqref{eq:srk} only queries the gradient of the potential,
% has the same per-iteration cost as the EM scheme
% , and improves
% the best available \wtwo-rate of LMC in the same setting
% from $\tilde{\mathcal{O}}(d \epsilon^{-1})$ to $\tilde{\mathcal{O}}(d \epsilon^{-2/3})$.
% Remarkably, the dimension dependence stays the same.

% after:
We emphasize that the 1.5 SRK scheme \eqref{eq:srk} only queries the gradient of the potential and improves 
the best available \wtwo-rate of LMC in the same setting
from $\tilde{\mathcal{O}}(d \epsilon^{-1})$ to $\tilde{\mathcal{O}}(d \epsilon^{-2/3})$,
with merely two extra gradient evaluations per iteration.
Remarkably, the dimension dependence stays the same.

\subsection{Sampling from Non-Convex Potentials with It\^o Diffusions}
\label{subsubsec:srk-nonconvex}
For the Langevin diffusion, the conclusions of Theorem~\ref{theo:master} only apply to distributions with strongly convex potentials, as exponential \wtwo-contraction of the Langevin diffusion is equivalent to strong convexity of the potential.
This shortcoming can be addressed using a non-constant diffusion coefficient which allows us to
sample from non-convex potentials using uniformly dissipative candidate diffusions. 
Below, we use a mean-square order 1.0 SRK scheme for general diffusions~\cite{rossler2010runge} and achieve an improved convergence rate compared to sampling with the EM scheme. 

We refer to the sampling algorithm as SRK-ID, which has the following update rule:
\eqn{
\tH_1^{(i)} &= \tX_k + \ssum_{j=1}^m \sigma_l(\tX_k) \frac{I_{(j,i)}}{\sqrt{h}}, \quad\quad
\tH_2^{(i)} = \tX_k - \ssum_{j=1}^m \sigma_l(\tX_k) \frac{I_{(j,i)}}{\sqrt{h}}, \\
\tX_{k+1} &= 
    \tX_k + h b(\tX_k)  + \ssum_{i=1}^m \sigma_i(\tX_k) I_{(i)} + 
            \frac{\sqrt{h}}{2} \ssum_{i=1}^m
        \big(
            \sigma_i (\tH_1^{(i)}) - \sigma_i (\tH_2^{(i)})
        \big), \numberthis \label{eq:srk_id}
}
where 
$
\text{
  \footnotesize
  $
    I_{(i)} = \sint_{t_k}^{t_{k+1}} \dB_s^{(i)}
  $
}$,
$
\text{
  \footnotesize
  $I_{(j,i)} = \sint_{t_k}^{t_{k+1}} \sint_{t_k}^{s} \dB_u^{(j)} \dB_s^{(i)}$
}
$.
% and 
% $
% \text{
%   \footnotesize
%   $
%     \{B_t^{(i)}\}_{t\ge0}
%   $
% }$ denotes the $i$th dimension of $\{B_t\}_{t\ge 0}$.
We note that schemes of higher order exist for general diffusions, but they typically require 
advanced approximations of iterated It\^o integrals of the form 
$
\text{
  \footnotesize
  $
    \int_0^{t_0} \cdots \int_0^{t_{n-1}} \dB_{t_n}^{(k_n)} \cdots \dB_{t_1}^{(k_1)}
  $
}$.
\begin{theo}[SRK-ID] \label{theo:srk_id}
  For a uniformly dissipative diffusion with invariant measure $\nu_*$, Lipschitz drift and diffusion coefficients that have Lipschitz gradients, 
  assume that the diffusion coefficient further satisfies the sublinear growth condition
% \eq{
%     \normop{\sigma(x)} \le \pi_{1,1}(\sigma)
%         \bracks{1 + \normtwo{x}^{1/2}},
%     \quad \text{for all} \; x \in \R^d,
%   }
$
  \text{
    \footnotesize
    $
    \normop{\sigma(x)} \le \pi_{1,1}(\sigma) \bigl(1 + \normtwo{x}^{1/2} \bigr)
    $
  }
$
for all $x \in \R^d$.
  % \todo{Isn't this the definition of $\pi_{1,1}$?  Is the assumption that $\pi_{1,1}$ is finite?}
  % \XL{Maybe call this ``square-root'' growth condition in the text just to re-emphasize?}
  % % \murat{We probably only need the op-norm of a(x) to grow linearly. Why need $\forall n$??}
  Let $\nu_k$ be the distribution of the $k$th Markov chain iterate
  defined by \eqref{eq:srk_id} starting from the dirac measure $\nu_0 = \delta_{x_0}$.
  Then for a sufficiently small step size, iterates of
  the 1.0 SRK scheme have uniform local deviation orders $(1.5, 2.0)$, and
  $W_2(\nu_k, \nu^*)$ converges within $\epsilon$ error in $\tilde{\mathcal{O}}(d^{3/4} m^{2} \epsilon^{-1})$
iterations.
\end{theo}
The proof is given in Appendix~\ref{app:srk_id} where 
we present explicit constants. We note that the dimension dependence in this case is only better than that of EM 
due to the extra growth condition on the diffusion. The extra $m$-dependence comes from the $2m$ evaluations of the 
diffusion coefficient at $\scriptstyle \tH_1^{(i)}$ and $\scriptstyle \tH_2^{(i)}$ ($i=1, \dots, m$). 
% For the diffusion coefficient, we use the Frobenius norm for the 
% Lipschitz and growth constants which could potentially hide the $d$-dependence. However, 
% since all constants are explicit, one may easily convert all bounds to be based on the operator norm 
% using the pessimistic inequality $\normf{\cdot} \le ( d^{1/2} + m^{1/2} ) \normop{\cdot}$.
In the above theorem, we use the Frobenius norm for the 
Lipschitz and growth constants for the diffusion coefficient 
which potentially hides dimension dependence. One may 
convert all bounds to be based on the operator norm 
% using the pessimistic inequality $\normf{\sigma(x)} \le ( d^{1/2} + m^{1/2} ) \normop{\sigma(x)}$ for all $x \in \R^d$
% then the convergence rate is expressed as $\tilde{\mathcal{O}}(d^3 m^2 \epsilon^{-2})$.
with our constants given in the Appendix. 
% \murat{Write the bound after the conversion.} 

In practice, accurately simulating both the iterated It\^o integrals $I_{(j,i)}$
and the Brownian motion increments $I_{(i)}$ simultaneously is difficult.
% Instead, one can approximate by truncating an infinite series; comments on this in Appendix~\ref{app:srk-id}.
We comment on two possible approximations based on truncating an infinite series in Appendix~\ref{app:srk-id}.

%%% Local Variables:
%%% mode:latex
%%% TeX-master: "./main.tex"
%%% End:

==> srk_arxiv_arXiv/utils/mathdef.tex <==
\newtheorem{defi}{Definition}
\newtheorem*{defi*}{Definition}
\numberwithin{defi}{section}
\newtheorem{fact}[defi]{Fact}
\newtheorem{algo}[defi]{Algorithm}
\newtheorem{cond}[defi]{Condition}
\newtheorem{prop}[defi]{Proposition}


\newtheorem{lemm}{Lemma}
\newtheorem{theo}[lemm]{Theorem}
\newtheorem{coro}[lemm]{Corollary}

\theoremstyle{remark}
\newtheorem*{remark}{\textbf{Remark}}

\theoremstyle{definition}
\newtheorem{exam}{\textbf{Example}}

\newcommand{\proofend}{\hfill$\Box$\vspace{2mm}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\define}{\stackrel{\mathrm{def}}{=}}
\newcommand{\argmin}{\mathop{\mathrm{argmin\,}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax\,}}}
\newcommand{\rank}[1]{\mathrm{rank}\left(#1\right)}
\newcommand{\tr}[1]{\mathrm{tr}(#1)}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\sinc}{\mathrm{sinc}\;}
\newcommand{\unorm}[1]{\|#1\|}
\newcommand{\unorms}[1]{\unorm{#1}^2}
\newcommand{\inner}[2]{\langle #1,#2\rangle}
\newcommand{\iid}{\stackrel{\mathrm{i.i.d.}}{\sim}}
\newcommand{\indep}{\mathop{\perp\!\!\!\perp}}

\newcommand{\pnu}{p}
\newcommand{\pde}{p'}
\newcommand{\Pnu}{P}
\newcommand{\Pde}{P'}
\newcommand{\pmix}{q_\alpha}
\newcommand{\numparams}{n}


\newcommand{\mathbbC}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\mathbbN}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\mathbbS}{\mathbb{S}}

\newcommand{\boldzero}{{\boldsymbol{0}}}
\newcommand{\boldone}{{\boldsymbol{1}}}

\newcommand{\boldA}{{\boldsymbol{A}}}
\newcommand{\boldB}{{\boldsymbol{B}}}
\newcommand{\boldC}{{\boldsymbol{C}}}
\newcommand{\boldD}{{\boldsymbol{D}}}
\newcommand{\boldE}{{\boldsymbol{E}}}
\newcommand{\boldF}{{\boldsymbol{F}}}
\newcommand{\boldG}{{\boldsymbol{G}}}
\newcommand{\boldH}{{\boldsymbol{H}}}
\newcommand{\boldI}{{\boldsymbol{I}}}
\newcommand{\boldJ}{{\boldsymbol{J}}}
\newcommand{\boldK}{{\boldsymbol{K}}}
\newcommand{\boldL}{{\boldsymbol{L}}}
\newcommand{\boldM}{{\boldsymbol{M}}}
\newcommand{\boldN}{{\boldsymbol{N}}}
\newcommand{\boldO}{{\boldsymbol{O}}}
\newcommand{\boldP}{{\boldsymbol{P}}}
\newcommand{\boldQ}{{\boldsymbol{Q}}}
\newcommand{\boldR}{{\boldsymbol{R}}}
\newcommand{\boldS}{{\boldsymbol{S}}}
\newcommand{\boldT}{{\boldsymbol{T}}}
\newcommand{\boldU}{{\boldsymbol{U}}}
\newcommand{\boldV}{{\boldsymbol{V}}}
\newcommand{\boldW}{{\boldsymbol{W}}}
\newcommand{\boldX}{{\boldsymbol{X}}}
\newcommand{\boldY}{{\boldsymbol{Y}}}
\newcommand{\boldZ}{{\boldsymbol{Z}}}
\newcommand{\bW}{{\boldsymbol{W}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bY}{{\boldsymbol{Y}}}

\newcommand{\bolda}{{\boldsymbol{a}}}
\newcommand{\boldb}{{\boldsymbol{b}}}
\newcommand{\boldc}{{\boldsymbol{c}}}
\newcommand{\boldd}{{\boldsymbol{d}}}
\newcommand{\bolde}{{\boldsymbol{e}}}
\newcommand{\boldf}{{\boldsymbol{f}}}
\newcommand{\boldg}{{\boldsymbol{g}}}
\newcommand{\boldh}{{\boldsymbol{h}}}
\newcommand{\boldi}{{\boldsymbol{i}}}
\newcommand{\boldj}{{\boldsymbol{j}}}
\newcommand{\boldk}{{\boldsymbol{k}}}
\newcommand{\boldl}{{\boldsymbol{l}}}
\newcommand{\boldm}{{\boldsymbol{m}}}
\newcommand{\boldn}{{\boldsymbol{n}}}
\newcommand{\boldo}{{\boldsymbol{o}}}
\newcommand{\boldp}{{\boldsymbol{p}}}
\newcommand{\boldq}{{\boldsymbol{q}}}
\newcommand{\boldr}{{\boldsymbol{r}}}
\newcommand{\bolds}{{\boldsymbol{s}}}
\newcommand{\boldt}{{\boldsymbol{t}}}
\newcommand{\boldu}{{\boldsymbol{u}}}
\newcommand{\boldv}{{\boldsymbol{v}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bz}{{\boldsymbol{z}}}


\newcommand{\boldztr}{\boldz^{\mathrm{tr}}}
\newcommand{\boldzte}{\boldz^{\mathrm{te}}}


\newcommand{\boldalpha}{{\boldsymbol{\alpha}}}
\newcommand{\boldbeta}{{\boldsymbol{\beta}}}
\newcommand{\boldgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bolddelta}{{\boldsymbol{\delta}}}
\newcommand{\boldepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\boldzeta}{{\boldsymbol{\zeta}}}
\newcommand{\boldeta}{{\boldsymbol{\eta}}}
\newcommand{\boldtheta}{{\boldsymbol{\theta}}}
\newcommand{\boldiota}{{\boldsymbol{\iota}}}
\newcommand{\boldkappa}{{\boldsymbol{\kappa}}}
\newcommand{\boldlambda}{{\boldsymbol{\lambda}}}
\newcommand{\boldmu}{{\boldsymbol{\mu}}}
\newcommand{\boldnu}{{\boldsymbol{\nu}}}
\newcommand{\boldxi}{{\boldsymbol{\xi}}}
\newcommand{\boldpi}{{\boldsymbol{\pi}}}
\newcommand{\boldrho}{{\boldsymbol{\rho}}}
\newcommand{\boldsigma}{{\boldsymbol{\sigma}}}
\newcommand{\boldtau}{{\boldsymbol{\tau}}}
\newcommand{\boldupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\boldphi}{{\boldsymbol{\phi}}}
\newcommand{\boldchi}{{\boldsymbol{\chi}}}
\newcommand{\boldpsi}{{\boldsymbol{\psi}}}
\newcommand{\boldomega}{{\boldsymbol{\omega}}}
\newcommand{\boldGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\boldDelta}{{\boldsymbol{\Delta}}}
\newcommand{\boldTheta}{{\boldsymbol{\Theta}}}
\newcommand{\boldLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\boldXi}{{\boldsymbol{\Xi}}}
\newcommand{\boldPi}{{\boldsymbol{\Pi}}}
\newcommand{\boldSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\boldUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\boldPhi}{{\boldsymbol{\Phi}}}
\newcommand{\boldPsi}{{\boldsymbol{\Psi}}}
\newcommand{\boldOmega}{{\boldsymbol{\Omega}}}
\newcommand{\boldvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\boldvartheta}{{\boldsymbol{\vartheta}}}
\newcommand{\boldvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\boldvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\boldvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\boldvarphi}{{\boldsymbol{\varphi}}}
 
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\boldcalZ}{{\bm \calZ}}
\newcommand{\boldcalY}{{\bm \calY}}
\newcommand{\boldcalB}{{\bm \calB}}

\newcommand{\calXtr}{{\mathcal{X}^{\mathrm{tr}}}}
\newcommand{\calYtr}{{\mathcal{Y}^{\mathrm{tr}}}}
\newcommand{\calXte}{{\mathcal{X}^{\mathrm{te}}}}
\newcommand{\calYte}{{\mathcal{Y}^{\mathrm{te}}}}

\newcommand{\thetah}{{\widehat{\theta}}}
\newcommand{\thetat}{{\widetilde{\theta}}}
\newcommand{\boldthetah}{{\widehat{\boldtheta}}}
\newcommand{\boldthetat}{{\widetilde{\boldtheta}}}
\newcommand{\boldzetah}{{\widehat{\boldzeta}}}
\newcommand{\calAh}{{\widehat{\calA}}}
\newcommand{\boldEh}{{\widehat{\boldE}}}
\newcommand{\boldGh}{{\widehat{\boldG}}}
\newcommand{\boldUh}{{\widehat{\boldU}}}
\newcommand{\Eh}{{\widehat{E}}}
\newcommand{\jh}{{\widehat{j}}}
\newcommand{\boldbetah}{{\widehat{\boldbeta}}}
\newcommand{\boldbetat}{{\widetilde{\boldbeta}}}

\newcommand{\mathrmd}{{\mathrm{d}}}
\newcommand{\longrightarrowD}{\stackrel{\mathrm{D}}{\longrightarrow}}

\newcommand{\domainx}{\calX}
\newcommand{\domainy}{\calY}
\newcommand{\domainz}{\calZ}
\newcommand{\inputdim}{d}
\newcommand{\reducedim}{m}
\newcommand{\reducedimh}{\widehat{\reducedim}}
\newcommand{\ntask}{m}
\newcommand{\nmix}{c}
\newcommand{\inputdimx}{\inputdim_{\mathrm{x}}}
\newcommand{\inputdimy}{\inputdim_{\mathrm{y}}}
\newcommand{\inputdimz}{\inputdim_{\mathrm{z}}}

\newcommand{\ratiosymbol}{r}
\newcommand{\ratio}{\ratiosymbol}
\newcommand{\ratioh}{\widehat{\ratiosymbol}}
\newcommand{\ratiomodel}{\ratiosymbol_{\alpha}}
\newcommand{\relratio}{\ratio_{\alpha}}

\newcommand{\densitysymbol}{p}
\newcommand{\cumulativesymbol}{P}
\newcommand{\density}{\densitysymbol^\ast}
\newcommand{\densitynu}{\densitysymbol_{\mathrm{te}}^\ast}
\newcommand{\densityde}{\densitysymbol_{\mathrm{de}}^\ast}
\newcommand{\densitydet}{\widetilde{\densitysymbol}_{\mathrm{de}}^\ast}
\newcommand{\cumulativede}{\cumulativesymbol_{\mathrm{de}}^\ast}
\newcommand{\cumulativenu}{\cumulativesymbol_{\mathrm{te}}^\ast}
\newcommand{\cumulativedeh}{\widehat{\cumulativesymbol}_{\mathrm{de}}}
\newcommand{\densityh}{\widehat{\densitysymbol}}
\newcommand{\densityt}{\widetilde{\densitysymbol}}
\newcommand{\densitynuh}{\widehat{\densitysymbol}_{\mathrm{te}}}
\newcommand{\densitydeh}{\widehat{\densitysymbol}_{\mathrm{de}}}
\newcommand{\densitymodel}{\densitysymbol}
\newcommand{\prior}{\pi}
\newcommand{\posterior}{\densitysymbol}
\newcommand{\evidence}{\densitysymbol}

\newcommand{\xy}{\mathrm{xy}}
\newcommand{\zy}{\mathrm{zy}}
\newcommand{\x}{\boldsymbol{x}}
\newcommand{\y}{\boldsymbol{y}}


\newcommand{\ptr}{p_{\mathrm{tr}}}
\newcommand{\pte}{p_{\mathrm{te}}}
\newcommand{\pxy}{p_{\mathrm{x,y}}}
\newcommand{\pzy}{p_{\mathrm{z,y}}}
\newcommand{\px}{p_{\mathrm{x}}}
\newcommand{\pz}{p_{\mathrm{z}}}
\newcommand{\py}{p_{\mathrm{y}}}
\newcommand{\boldxtr}{\boldx^{\mathrm{tr}}}
\newcommand{\boldxte}{\boldx^{\mathrm{te}}}
\newcommand{\xtr}{x^{\mathrm{tr}}}
\newcommand{\xte}{x^{\mathrm{te}}}
\newcommand{\ytr}{y^{\mathrm{tr}}}
\newcommand{\yte}{y^{\mathrm{te}}}
\newcommand{\epsilontr}{\epsilon^{\mathrm{tr}}}
\newcommand{\epsilonte}{\epsilon^{\mathrm{te}}}
\newcommand{\ntr}{n}
\newcommand{\nte}{n_{\mathrm{te}}}
\newcommand{\nteu}{n_{\mathrm{te}}'}
\newcommand{\ntep}{n_{\mathrm{te}}}
\newcommand{\densitytr}{\densitysymbol_{\mathrm{tr}}^\ast}
\newcommand{\densityte}{\densitysymbol_{\mathrm{te}}^\ast}
\newcommand{\Xtr}{X^{\mathrm{tr}}}
\newcommand{\Xte}{X^{\mathrm{te}}}
\newcommand{\boldXtr}{\boldX^{\mathrm{tr}}}
\newcommand{\boldXte}{\boldX^{\mathrm{te}}}
\newcommand{\boldytr}{\boldy^{\mathrm{tr}}}
\newcommand{\boldyte}{\boldy^{\mathrm{te}}}
\newcommand{\Gen}{G}
\newcommand{\Genh}{\widehat{\Gen}}

\newcommand{\boldxnu}{\boldx^{\mathrm{te}}}
\newcommand{\boldxde}{\boldx^{\mathrm{tr}}}
\newcommand{\boldxt}{\widetilde{\boldx}}

\newcommand{\boldunu}{\boldu^{\mathrm{te}}}
\newcommand{\boldude}{\boldu^{\mathrm{tr}}}
\newcommand{\boldvnu}{\boldv^{\mathrm{te}}}
\newcommand{\boldvde}{\boldv^{\mathrm{tr}}}
\newcommand{\boldunuh}{\widehat{\boldu}^{\mathrm{te}}}
\newcommand{\boldudeh}{\widehat{\boldu}^{\mathrm{tr}}}
\newcommand{\unu}{u^{\mathrm{te}}}
\newcommand{\ude}{u^{\mathrm{tr}}}

\newcommand{\nde}{n_{\mathrm{tr}}}
\newcommand{\nnu}{n_{\mathrm{te}}}
\newcommand{\nsample}{n}

\newcommand{\nparam}{b}
\newcommand{\nparamm}{t}
\newcommand{\nclass}{c}
\newcommand{\ndet}{\widetilde{n}_{\mathrm{tr}}}

\newcommand{\data}{D}
\newcommand{\datanu}{D^{\mathrm{te}}}
\newcommand{\datade}{D^{\mathrm{tr}}}

\newcommand{\boldratiosymbol}{\boldr}
\newcommand{\boldratio}{\boldratiosymbol^\ast}
\newcommand{\boldratiomodel}{{\boldratiosymbol}}
\newcommand{\boldratiode}{\boldratiosymbol_{\mathrm{tr}}^\ast}
\newcommand{\boldrationu}{\boldratiosymbol_{\mathrm{te}}^\ast}
\newcommand{\boldratioh}{\widehat{\boldratiosymbol}}
\newcommand{\boldratiodeh}{\boldratioh_{\mathrm{tr}}}
\newcommand{\boldrationuh}{\boldratioh_{\mathrm{te}}}
\newcommand{\boldratiodemodel}{\boldratiomodel_{\mathrm{tr}}}
\newcommand{\boldrationumodel}{\boldratiomodel_{\mathrm{te}}}
\newcommand{\boldPhide}{\boldPhi_{\mathrm{tr}}}
\newcommand{\boldPhinu}{\boldPhi_{\mathrm{te}}}
\newcommand{\boldPside}{\boldPsi_{\mathrm{tr}}}
\newcommand{\boldPsinu}{\boldPsi_{\mathrm{te}}}

\newcommand{\Bregman}{\mathrm{BR}}
\newcommand{\fdivergence}{\mathrm{ASC}}

\newcommand{\function}{f^\ast}
\newcommand{\functionmodel}{f}
\newcommand{\functionh}{\widehat{f}}

\newcommand{\xde}{x^{\mathrm{tr}}}
\newcommand{\xdet}{\widetilde{x}^{\mathrm{tr}}}
\newcommand{\xnu}{x^{\mathrm{te}}}
\newcommand{\zde}{z^{\mathrm{tr}}}
\newcommand{\boldxdet}{\widetilde{\boldx}^{\mathrm{tr}}}
\newcommand{\boldxnut}{\widetilde{\boldx}^{\mathrm{te}}}
\newcommand{\etade}{\eta^{\mathrm{tr}}}
\newcommand{\etanu}{\eta^{\mathrm{te}}}
\newcommand{\boldepsilonde}{\boldepsilon^{\mathrm{tr}}}
\newcommand{\boldepsilondet}{\widetilde{\boldepsilon}^{\mathrm{tr}}}
\newcommand{\epsilonde}{\epsilon^{\mathrm{tr}}}
\newcommand{\epsilonnu}{\epsilon^{\mathrm{te}}}
\newcommand{\epsilondeh}{\widehat{\epsilon}^{\mathrm{tr}}}
\newcommand{\epsilondet}{\widetilde{\epsilon}^{\mathrm{tr}}}
\newcommand{\boldrde}{\boldr^{\mathrm{tr}}}
\newcommand{\boldrnu}{\boldr^{\mathrm{te}}}
\newcommand{\Ade}{A^{\mathrm{tr}}}
\newcommand{\Anu}{A^{\mathrm{te}}}
\newcommand{\Xde}{X^{\mathrm{tr}}}
\newcommand{\Xdet}{\widetilde{X}^{\mathrm{tr}}}
\newcommand{\Xnu}{X^{\mathrm{te}}}
\newcommand{\boldXde}{\boldX^{\mathrm{tr}}}
\newcommand{\boldXdet}{\widetilde{\boldX}^{\mathrm{tr}}}
\newcommand{\boldXnu}{\boldX^{\mathrm{te}}}
\newcommand{\boldGde}{\boldG^{\mathrm{tr}}}
\newcommand{\boldGnu}{\boldG^{\mathrm{te}}}
\newcommand{\boldAde}{\boldA^{\mathrm{tr}}}
\newcommand{\boldAnu}{\boldA^{\mathrm{te}}}
\newcommand{\boldKdede}{\boldK_{\mathrm{tr},\mathrm{tr}}}
\newcommand{\boldKdenu}{\boldK_{\mathrm{tr},\mathrm{te}}}
\newcommand{\boldKde}{\boldK_{\mathrm{tr}}}
\newcommand{\boldKnu}{\boldK_{\mathrm{te}}}
\newcommand{\boldyde}{\boldy^{\mathrm{tr}}}
\newcommand{\boldydet}{\widetilde{\boldy}^{\mathrm{tr}}}
\newcommand{\Kdede}{K_{\mathrm{tr},\mathrm{tr}}}
\newcommand{\Kdenu}{K_{\mathrm{tr},\mathrm{te}}}
\newcommand{\Kde}{K_{\mathrm{tr}}}
\newcommand{\yde}{y^{\mathrm{tr}}}
\newcommand{\ydet}{\widetilde{y}^{\mathrm{tr}}}
\newcommand{\ynu}{y^{\mathrm{te}}}
\newcommand{\yh}{\widehat{y}}
\newcommand{\ynuh}{\widehat{y}^{\mathrm{te}}}
\newcommand{\calXde}{\calX^{\mathrm{tr}}}
\newcommand{\calYde}{\calY^{\mathrm{tr}}}
\newcommand{\calZde}{\calZ^{\mathrm{tr}}}
\newcommand{\calXnu}{\calX^{\mathrm{te}}}
\newcommand{\calYnu}{\calY^{\mathrm{te}}}
\newcommand{\calZnu}{\calZ^{\mathrm{te}}}
\newcommand{\calZt}{\widetilde{\calZ}}

\newcommand{\Pb}{{P^{\ast}}'}
\newcommand{\Pa}{P^\ast}
\newcommand{\pb}{{p^{\ast}}'}
\newcommand{\pa}{p^\ast}
\newcommand{\nb}{n'}
\newcommand{\na}{n}
\newcommand{\calXb}{\calX'}
\newcommand{\calXa}{\calX}
\newcommand{\calXbt}{\widetilde{\calX}'}
\newcommand{\calXat}{\widetilde{\calX}}
\newcommand{\boldxb}{\boldx'}
\newcommand{\boldxa}{\boldx}
\newcommand{\boldHhde}{{\widehat{\boldH}}}
\newcommand{\boldhhde}{{\widehat{\boldh}}'}
\newcommand{\boldhhnu}{{\widehat{\boldh}}}
\newcommand{\boldGhde}{{\widehat{\boldG}}}
\newcommand{\boldghde}{{\widehat{\boldg}}'}
\newcommand{\boldghnu}{{\widehat{\boldg}}}
\newcommand{\nn}{\overline{n}}

\newcommand{\boldTh}{{\widehat{\boldT}}}
\newcommand{\boldgh}{{\widehat{\boldg}}}
\newcommand{\boldHh}{{\widehat{\boldH}}}
\newcommand{\boldhh}{{\widehat{\boldh}}}
\newcommand{\boldBh}{{\widehat{\boldB}}}
\newcommand{\Hh}{{\widehat{H}}}
\newcommand{\hh}{{\widehat{h}}}
\newcommand{\boldHt}{{\widetilde{\boldH}}}
\newcommand{\boldht}{{\widetilde{\boldh}}}
\newcommand{\boldDt}{{\widetilde{\boldD}}}
\newcommand{\boldWt}{{\widetilde{\boldW}}}
\newcommand{\boldXt}{{\widetilde{\boldX}}}
\newcommand{\Wt}{{\widetilde{W}}}
\newcommand{\Dt}{{\widetilde{D}}}
\newcommand{\Qt}{{\widetilde{Q}}}
\newcommand{\Qh}{{\widehat{Q}}}
\newcommand{\Ht}{{\widetilde{H}}}
\newcommand{\Xt}{{\widetilde{X}}}
\newcommand{\Jh}{\widehat{J}}
\newcommand{\Jt}{\widetilde{J}}
\newcommand{\Vh}{\widehat{V}}
\newcommand{\Fh}{\widehat{F}}
\newcommand{\Gh}{\widehat{G}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\KLh}{\widehat{\KL}}
\newcommand{\KLt}{\widetilde{\KL}}
\newcommand{\boldxih}{\widehat{\boldxi}}
\newcommand{\boldalphah}{\widehat{\boldalpha}}
\newcommand{\boldalphat}{\widetilde{\boldalpha}}
\newcommand{\alphah}{\widehat{\alpha}}
\newcommand{\sigmah}{{\widehat{\sigma}}}
\newcommand{\lambdah}{{\widehat{\lambda}}}

\newcommand{\boldSb}{\boldS^{\mathrm{b}}}
\newcommand{\boldSw}{\boldS^{\mathrm{w}}}
\newcommand{\boldWb}{\boldW^{\mathrm{b}}}
\newcommand{\boldWw}{\boldW^{\mathrm{w}}}
\newcommand{\Wb}{W^{\mathrm{b}}}
\newcommand{\Ww}{W^{\mathrm{w}}}
\newcommand{\boldSlb}{\boldS^{\mathrm{lb}}}
\newcommand{\boldSlw}{\boldS^{\mathrm{lw}}}
\newcommand{\boldWlb}{\boldW^{\mathrm{lb}}}
\newcommand{\boldWlw}{\boldW^{\mathrm{lw}}}
\newcommand{\Wlb}{W^{\mathrm{lb}}}
\newcommand{\Wlw}{W^{\mathrm{lw}}}
\newcommand{\weight}{w}
\newcommand{\weighth}{\widehat{w}}


\newcommand{\resample}{\zeta}
\newcommand{\CEVOW}{\textrm{CV}_\textrm{W}}
\newcommand{\PCEVOW}{\textrm{PCV}_\textrm{W}}
\newcommand{\CEVOO}{\textrm{CV}_\textrm{O}}
\newcommand{\PCEVOO}{\textrm{PCV}_\textrm{O}}
\newcommand{\FEVOW}{\textrm{FV}_\textrm{W}}
\newcommand{\PFEVOW}{\textrm{PFV}_\textrm{W}}
\newcommand{\FEBVOW}{\textrm{FBV}_\textrm{OW}}
\newcommand{\PFEBVOW}{\textrm{PFBV}_\textrm{OW}}
\newcommand{\ALICE}{\textrm{ALICE}}
\newcommand{\PALICE}{\textrm{PALICE}}

\newcommand{\model}{M}
\newcommand{\GhatAL}{\Genh^{(AL)}}
\newcommand{\GhatMS}{\Genh^{(MS)}}
\newcommand{\GhatuCEAL}{\Genh^{(EAL)}}
\newcommand{\GhatCEAL}{\Genh^{(nEAL)}}

\newcommand{\hatgn}{\widehat{g}_n}
\newcommand{\gnstar}{g_n^*}
\newcommand{\alzn}{\alpha_0^n}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\gzn}{\ratio}
\newcommand{\Gconv}{\mathcal{G}^{(\mathrm{c})}}



